Efficiency-Risk Tradeoffs in Dynamic Oligopoly Markets - with application to electricity markets

In this paper, we examine in an abstract framework, how a tradeoff between efficiency and robustness arises in different dynamic oligopolistic market architectures. We consider a market in which there is a monopolistic resource provider and agents that enter and exit the market following a random process. Self-interested and fully rational agents dynamically update their resource consumption decisions over a finite time horizon, under the constraint that the total resource consumption requirements are met before each individual's deadline. We then compare the statistics of the stationary aggregate demand processes induced by the non-cooperative and cooperative load scheduling schemes. We show that although the non-cooperative load scheduling scheme leads to an efficiency loss - widely known as the "price of anarchy" - the stationary distribution of the corresponding aggregate demand process has a smaller tail. This tail, which corresponds to rare and undesirable demand spikes, is important in many applications of interest. On the other hand, when the agents can cooperate with each other in optimizing their total cost, a higher market efficiency is achieved at the cost of a higher probability of demand spikes. We thus posit that the origins of endogenous risk in such systems may lie in the market architecture, which is an inherent characteristic of the system.

==> _region_.tex <==
\message{ !name(general_L_pricing_section1.tex)}
\message{ !name(general_L_pricing_section1.tex) !offset(-2) }
% \tc{red}{
% LTI here:\\ 
% introduce the substitute measure, and approximation of continuous arrival
% \\
% leave the relaxation of deadline and calculate the bound to next section
% }

%   \section{General $L$ Analysis: Pricing}
\chapter{General $L$ Analysis: Pricing}
\label{sec:pricing}


As illustrated in Figure~\ref{fig:sys_diag_1}, the agents who make their load scheduling
decisions can be viewed as a full state feedback controller, the control signal $\mb u(t)$
is fed back to the plant and affects the system state evolution following
(\ref{eq:state-evolve-gen1}) and (\ref{eq:state-evolve-gen2}), and the system output is the
aggregate demand process $\{U(t):t\in\mbb Z\}$.
 %
In the case with $L=2$, even when the existing agents adopt a linear strategy, the system
dynamics is not linear since the type $2$ agents $(2,2)_t$ do not arrive at every period
$t$.
%
For a general $L$, the load scheduling strategy, which is determined under a specific
market architecture, does not form a linear time-invariant feedback controller.
% If a symmetric linear strategy is adopted by the agents that are present in the market,
% the system follows a jump linear dynamics and the mode switching events are determined by
% the Bernoulli arrival process.
% %
% As an example, the jump linear system diagram is shown in
% Figure~\ref{fig:jump_linear_combo}.
% More generally, for $L$ types of agents, the existence state is a $D_c$-dimensional
% vector, where $D_c = L(L+1)/2$.  There are in total $2^{D_c}$ possible existence
% states.  Assuming that linear strategies are adopted and the instantaneous demand from
% agent $(l,\tau)_t$ equals $u_{(l,\tau)}(t) = \mb F_{(l,\tau)}\mb x(t)$, each of the
% existence state corresponds to a linear mode. The Bernoulli arrival process together
% with the evolution of existence state lead to mode change.  \small even for $L=3$ is
% very messy Take $L=3$, and $q_l=q$ for all $l\in\mathcal L$ as an example, the
% transition among different mode is depicted in Figure~\ref{fig:jump_linear_combo} (b).
% It has $2^6 = 64$ states... very messy when the transition probabilities are specified.
%
%Moreover, for the general case,
The non-linearity as a result of the Bernoulli processes complicates the analysis, and
there is no explicit solution to the equilibrium load scheduling strategy under marginal
cost pricing in both the cooperative and the non-cooperative scheme.
% \begin{figure}[h!]  \centering
%   \includegraphics[width = 0.6 \textwidth]{eps/jump_linear_combo.jpg}
%   \caption{Markov jumped linear system diagram, for $L=2$. There are two modes,
%     corresponding to the existence state of the new type 2 agent  $h_2 = 0$ and $h_2 = 1$.}
%   \label{fig:jump_linear_combo}
% \end{figure}

We realize that the main hurdle of analyzing the general $L$ case lies in the nonlinear
dynamics due to the intermittent agent arrivals.  To circumvent the problem we shall
introduce a modified system with surrogate performance measures, which resembles the
original system in the most essential ways and facilitates the analysis. The
results obtained in this LTI framework can provide us some insights on the original
non-linear system dynamics and the efficiency-risk tradeoffs.
%
The two key modifications are listed and interpreted as follows:
\begin{Modif}
  The agent arrival rate $\mb q= \mb 1$, namely agents of all types arrive at every
  period, so that $\mb h(t) = \mb 1$ and $\mb o(t) = \mb 1$ for all $t$.
  \label{modif:mod1}
\end{Modif}
\begin{Modif}
  The second moment $\mbb E[z_2(t)^2]$ of the aggregate backlog process $z_2(t) = \mb e' \mb
  x(t)$ is used as a substitute measure for risk.
  \label{modif:mod2}
\end{Modif}


%\tc{red}{justification:}
We focus on the case with $\mb q=1$, which is a reasonable approximation in the
regime of high arrival rate $\mb q$.
%
As discussed briefly at the end of
% Section~\ref{sec:numerical-results},
Chapter~\ref{sec:numerical-results},
there are two senarios where an aggregate demand spike can occur.
%
On one hand, the instantaneous aggregate demand will be driven up when the workload
realization $d_{l}(t)$ from either type of agent is extremely high, which corresponds to
the rare events of the load arrival processes. We classify this type of spikes to be
exogenous. Moreover, for bounded support of $\mb D_l$ and large enough constant $M$, the
exogenous shocks do not directly contribute to the risk measure.
%
On the other hand, an aggregate spike can also be produced endogenously when a high
backlog is built up and the agents with flexible loads, who can absorb the endogenous
shock, are absent in the market.
%
As an exmple, Figure~\ref{fig:whereSpikes1} shows the high correlations between demand
spikes and the event of high backlog state, as well as between demand spikes and the
absence of type 2 agents.
%
% In the following, we shall focus on the endogenously produced spikes, and the volatility
% of the aggregate backlog process, measured by its variance, will be used as a substitute
% risk measure.
%
%Notice that there is no contradiction between the first two modifications.
We examine the evolution of the backlog state in the regime where $\mb q$ is close to
$\mb 1$, and the equilibrium strategy will be similar to the case of $\mb q=\mb 1$;
however, absence of flexible load still happens exogenously with small probabilities, and
upon which occurrences a high backlog is turned into a demand spike. Therefore, the
volatility of the aggregate backlog state is used as a substitute measure for the risk of
spikes.
%


We also normalize the load arrival process so that the average load realization
$\boldsymbol{\mu}$, the average backlog state $\mbb E[\mb x(t)]$, and the average demand
$\mbb E[\mb u(t)]$, are all zero vectors. We also assume the load arrival process $\{\mb
d(t):t\in\mbb Z\}$ is an i.i.d. process.
% since a constant shift of aggregate demand in every period amounts to a constant shift in
% aggregate backlog.
In summary, the system diagram of the modified system with linear dynamics is shown in
Figure~\ref{fig:sys_diag_2}. The performance measures are the variance of the two outputs:
\begin{align}
  %\mb z(t) =
  \left[
      \begin{array}{c}
        z_1(t)
        \\
        z_2(t)
      \end{array}
    \right] =\left[
      \begin{array}{c}
        \mb e' \mb u(t)
        \\
        \mb e' \mb x(t)
      \end{array}
    \right]. \nonumber
\end{align}




%------------------------------------------------------------------------------------

% In the previous section, we have modified our problem so that it fits into an LTI
% framework. Fixing the marginal cost pricing rule, we showed that any load scheduling
% scheme cannot achieve better outcomes than that specified by the Pareto front in
% Proposition \ref{prop:three-way}.
%
From the system operator's view, we are interested in how agent decision making is shaped
by the market architecture, and how the architecture should be designed so that the
desired agent behavior is induced.
%
Usually many of the market architectural properties, for example the degree of
cooperation and risk sensitivity of the agents are given, and the system operator's only
freedom is to design the pricing rule.
%
In the following, we shall consider a non-cooperative setup within the LTI framework, and
examine the equilibrium load scheduling strategies under any linear pricing rule, which
rule will be decided by the system operator\footnote{ In
  Appendix~\ref{sec:conge-fee-degree}, we study another example where the system operator
  regulates the architectural property of ``degree of cooperation'' by imposing a
  ``congestion fee''.}.
%
In particular, we focus on the static linear pricing rules parameterized by coefficients
$\mb q_1$ and $\mb q_2$, in the form:
\begin{align}
  p(t) = \mb q_1'\mb x(t) + \mb q_2'\mb u(t).
  \label{eq:linear-pricing}
\end{align}
% \begin{enumerate}
% \item Static pricing, only depending on backlog $\mb x(t)$:
%   \[p(t) = \mb x(t)'\mb q\]  
% \item Static pricing, depending on $\mb x(t)$ and $\mb u(t)$:
%   \[p(t) = \mb x(t)'\mb q_1 + \mb u(t)' \mb q_2\]
% \item Dynamic pricing, with memory:
%   \[p(t) = \sum_{k=0}^{N-1} \mb x(t-k)'\mb q_{1, k} + \sum_{k=0}^{N-1} \mb u(t-k)'\mb
%   q_{2, k}\]
% \end{enumerate}
% where $\mb q$, $\mb q_1$, $\mb q_2$, and $\mb q_{i,k}$ are $D_c$ dimensional constant
% vectors.  is adaptive to the backlog state $\mb x(t)$ and instantaneous demand $\mb u(t)$
% We consider three cases as follows: In all cases, there exists a linear symmetric
% equilibrium. For the static cases , the linear load scheduling strategy is in the form of:% \[\mb u(t) = \mb F^* \mb x(t)\]
% and for the dynamic case, it is in the form of:
% \[\mb u(t) = \sum_{k = 0}^{N-1} \mb F^*_k \mb x(t-k)\]
The instantaneous demand decisions are made by individual agents under the deadline
constraints in a non-cooperative way.  We restrict ourselves to the linear symmetric
MPE, assuming that the load scheduling strategy, if exists, is in the following
form:
\begin{align}
  \mb u^*(t) = \mb F^* \mb x(t),
  \label{eq:consistency}
\end{align}
and we denote the $(l,\tau)$-th row of $\mb F^*$ by $\mb F_{(l,\tau)}^*\in\mbb R^{D_c}$. By
individual rationality, $u_{(l,\tau)}(t)$ is optimized by agent $(l,\tau)_t$ when he
dynamically updates his load scheduling decision, forming the rational expectation that
all other agents are adopting the equilibrium linear strategy as in
(\ref{eq:consistency}). More specifically, apply the one-shot deviation principle and we
have:
%
\begin{align}
  \fa (l,\tau)\in\mc C, \tx{if } \tau >1,
  \quad &u_{(l,\tau)}^*(t) %= \mb F_{(l,\tau)}^* \mb x(t)
  = \arg\min_{u\in\mbb R} \left\{ \mb p(t) u + \mbb E[ \sum_{k=1}^{\tau-1}\mb p(t+k) \mb
    F_{(l,\tau-k)}^* \mb x(t+k) ] \right\}
  \label{eq:IR-cons}
  \\
  \tx{subject to: }
  & \mb u(t) = \mb F^*\mb x(t) + \mb e_{(l,\tau)} (u - \mb F^*_{(l,\tau)}\mb x(t))
  \nonumber\\
  & \mb u(t+k) = \mb F^*\mb x(t+k), \ \ \fa k>0
  \nonumber\\
  & p(i) = \mb q_1'\mb x(i) + \mb q_2'\mb u(i), \ \ \fa i
  \nonumber\\
  & \mb x(i+1) = \mb R_1\mb x(i) + \mb R_2 \mb d(i) - \mb R_1\mb u(i), \ \ \fa i
  %\ \ \tx{for  } k = 2,\dots, \tau-1,  
  % &\qquad \mb x(t+1) = \mb R_1(\mb I - \mb F^*)\mb x(t) + \mb R_2 \mb d(t) + \mb R_1 \mb
  % e_{(l,\tau)}(\mb F^*_{(l,\tau)} \mb x(t) - u),
  % \\
  % &\qquad \mb x(t+k) = \mb R_1(\mb I - \mb F^*) \mb x(t+k-1) + \mb R_2 \mb d(t+k-1) \ \ \tx{for
  % } k = 2,\dots, \tau-1,   
  \nonumber\\
  \tx{if } \tau =1, \quad & u_{(l,\tau)}^*(t) = \mb e_{(l,\tau)}\mb x(t), \nonumber
\end{align}
where $\mb e_{(l,\tau)}$ is a $D_c$ dimensional vector with the only non-zero element
being $1$ at the $(l,\tau)$-th position. Moreover, at the symmetric equilibrium the
rational expectation should be consistent with the best response strategy, namely
(\ref{eq:consistency}) should be satisfied.


%= \mb F_{(l,\tau)}^* \mb x(t)

A direct application of the principle of optimality to  (\ref{eq:IR-cons}) leads to 
% Simplify the first order conditions of the rationality constraints in we have:
\begin{align}
\mb F^* = f_{(\mb q_1, \mb q_2)} (\mb F^*)
\label{eq:fixed-point-F-f}
\end{align}
For given coefficients $\mb q_1, \mb q_2$, the $(l,\tau)$-th row of the mapping $f_{(\mb
  q_1, \mb q_2)}:\mbb R^{D_c\times D_c}\to \mbb R^{D_c\times D_c}$ is specified as follows:
\begin{align}
    f_{(\mb q_1, \mb q_2)}(\mb F)_{(l,\tau)} = \left\{
    \begin{array}[]{ll}
     \mb e_{(l,\tau)}'
      & \tx{if } \tau=1,
      \\
    \frac{\mb e_{(l,\tau)}'\mb R_1' \mb A_{(l,\tau)}
        \Big(\mb R_1(\mb I - \mb F) + \mb R_1\mb e_{(l,\tau)}\mb F_{(l,\tau)} \Big)
        - \Big(\mb q_1' + \mb q_2'(\mb F-\mb e_{(l,\tau)}\mb F_{(l,\tau)}) \Big)}
      {\mb e_{(l,\tau)}'\mb R_1' \mb A_{(l,\tau)} \mb R_1\mb e_{(l,\tau)}  + 2 \mb e_{(l,\tau)}'\mb
        q_2}
      &\tx{if  } \tau >1,
    \end{array}
  \right.
  \label{eq:fixed-point-f-def}
\end{align}
where
\[ 
\mb A_{(l,\tau)} =\sum_{k=1}^{\tau-1}
\Big(\big (\mb R_1(\mb I - \mb F)\big)^{k-1}\Big)'
\Big(
(\mb q_1 + \mb F'\mb q_2) \mb F_{(l,\tau-k)}
+ \mb F_{(l,\tau-k)}'(\mb q_1' + \mb q_2 '\mb F)
\Big)
  \Big(\big (\mb R_1(\mb I - \mb F) \big)^{k-1}\Big).
\]
The highly nonlinear mapping $f_{(\mb q_1,\mb q_2)}$ is not a contraction.  Obtaining the
conditions on the parameters that guarantee the existence of a fixed point solution to
(\ref{eq:fixed-point-f-def}) is a challenging task. However, the equation still provides
a set of necessary conditions for the equilibrium strategies to satisfy.
%
An iteration algorithm with a carefully chosen initial guess will converge to such a
fixed point, and we will use numerical examples to show how the pricing parameter $\mb
q_1$ and $\mb q_2$ shift the equilibrium.


Instead, we shall examine some numerical results in the following and draw some guidelines
that the system operator should pay attention to when designning the pricing rule.
%

\tc{red}{ First, we consider the case with $L=3$. For the parameterized linear pricing
  rule given in (\ref{eq:linear-pricing}), we plot the Pareto front of the aggregate
  demand variance (-efficiency) and the aggregate backlog variance (risk) in
  Figure~\ref{fig:pricing-front-12}. We examine the pricing rules that lead to outcomes
  on the Pareto front, and we find that compared to the case of marginal cost pricing,
  the system operator can optimize the pricing rule to improve efficiency and reduce risk
  at the same time. Moreover, it shows that by putting a higher relative weight on the
  most urgent backlog state, i.e., higher $\mb q_1(2)/\mb q_1(1)$ and $\mb q_1(3)/\mb
  q_1(1)$, we can trade market efficiency with a lower risk along the Pareto front.
 \\
  Second, we examine the impact of the pricing rule sets on the location of the Pareto
  front. In Figure~\ref{fig:pricing-front-3}, we compare the Pareto front induced by the
  pricing rules in the form $p(t) = \mb q_1'\mb x(t) + \mb q_2'\mb u(t)$ and induced by
  the pricing rules in the form $p(t) = \sum_{i=0}^{1}\mb q_{1,i}'\mb x(t-i) +
  \sum_{i=0}^{1}\mb q_{2,i}'\mb u(t-i)$. We observe that by adopting a class of more
  general pricing rules, the system operator is able to push the Pareto front.
  }

\begin{Prop}[System operator's problem]
  \label{prop:operator-problem}

  Assume the system operator's utility function is increasing in efficiency and
  decreasing in risk, and in particular is linearly decreasing in both the volatility of
  aggregate demand and aggregate backlog as follows:
  \[J(\mbb E[z_1(t)^2], \mbb E[z_1(t)^2]) = -(\alpha_1\mbb E[z_1(t)^2] + \alpha_2 \mbb
  E[z_1(t)^2]).\]
%
  The system operator optimizes the parameterized pricing rule as defined in
  (\ref{eq:linear-pricing}) to maximizes its utility, and the optimal solution $(\mb
  q_1^*, \mb q_2^*)$ is given by solving the following problem:
  \begin{align}
    &\min_{\mb q_1, \mb q_2 \in\mbb R^{D_c}, \ \mb Q, \mb F\in \mbb R^{D_c\times D_c}}
    \alpha_1\mb e'\mb F_{(\mb q_1, \mb q_2)} \mb Q \mb F_{(\mb q_1, \mb q_2)}\mb e +
    \alpha_2\mb e'\mb Q\mb e
   \label{eq:system-operator-opt}
   \\
   &\tx{subject to: } \mb R_1 (\mb I-\mb F)\mb Q (\mb I-\mb F')\mb R_1'
   - \mb Q + \mb R_2\mb R_2'= \mb 0
   \label{eq:system-operator-opt-c1}\\
   &\qquad\qquad\ \mb F = f_{(\mb q_1, \mb q_2)}(\mb F)
   \label{eq:system-operator-opt-c2}
 \end{align}
 where $f_{(\mb q_1, \mb q_2)}$ is the mapping defined in (\ref{eq:fixed-point-f-def}).
\end{Prop}
\begin{Proof}
  Please refer to Appendix~\ref{prf:operator-problem}.
\end{Proof}








%<!-- don't delete these notes

%\subsubsection{modified system}
% In the modified system. Agents of every type arrive in each period, therefore
% \[\mb h(t) = \mb 1, \quad \mb z(t) = \mb 1\]
% the load realization at each period $t$ is denoted as
% \[\mb d(t) = [d_l(t):l\in\mathcal L]\]
% System state is the $D_c$ dimensional backlog state $\mb x(t)$ which evolves according to the
% following dynamics:
% \[\mb x(t+1) = \mb R_1\big(\mb x(t) - \mb u(t)\big) + \mb R_2 \mb d(t) \]
% where $\mb u(t)$ is the instantaneous demand vector.  The two objectives are aggregate demand
% volatility $\mbb E[(\mb e' \mb u(t))^2]$ and aggregate backlog volatility $\mbb E[(\mb e' \mb
% x(t))^2]$, which represent the measures of negative efficiency and risk, separately.



% \subsubsection{Equilibrium characterization}
% We specify the first order condition on $u$,
% \begin{align*}
%   0= \ \  &\mb x(t)'
%   \Big(\mb q_1 + (\mb F^* -\mb e_{(l,\tau)}\mb F_{(l,\tau)}^*)' \mb q_2
%   \Big) + 2 \mb e_{(l,\tau)}'\mb q_2 u -
%   \\
%   \ &\mb e_{(l,\tau)}' \mb R_1' \sum_{k = 1}^{\tau-1} \Big\{
%   \Big(\big( \mb R_1(\mb I - \mb F^*)\big)^{k-1}\Big )'
%   \Big( (\mb q_1 + \mb F^{*'}\mb q_2) \mb F_{(l,\tau-k)}^*
%   + \mb F_{(l,\tau-k)}^{*'}(\mb q_1' + \mb q_2 '\mb F^{*}) \Big)
%   \\ &
%   \Big(\big( \mb R_1(\mb I - \mb F^*) \big )^{k-1}\Big)
%   \Big\}  
%   \Big(\mb R_1(\mb I - \mb F^*)\mb x(t) + \mb R_1 \mb e_{(l,\tau)}(\mb F^*_{(l,\tau)} \mb x(t)
%   - u)\Big)  
% \end{align*} 
% Note that under the normalization assumption, $\mbb E[\mb d(t)] = \mb 0, (\fa t)$, we have that:
% \[
%  \mbb E[\mb x(t+k)] = \big( \mb R_1(\mb I - \mb F^*) \big)^{k-1} \mb x(t+k-1) 
% \]
% Solving the equation linear in $\mb x(t)$ and in $u$, we match the coefficients to obtain:
% \begin{align*}
%   u 
%   &= \frac{\mb e_{l,\tau)}'\mb R_1' \mb A_{(l,\tau)}
%     \Big(\mb R_1(\mb I - \mb F^*) + \mb R_1\mb e_{(l,\tau)}\mb F_{(l,\tau)}^* \Big)
%    - \Big(\mb q_1' + \mb q_2'(\mb F^*-\mb e_{(l,\tau)}\mb F_{(l,\tau)}^*) \Big)}
%   {\mb e_{(l,\tau)}'\mb R_1' \mb A_{(l,\tau)} \mb R_1\mb e_{(l,\tau)}  + 2 \mb e_{(l,\tau)}'\mb
%   q_2}
%   \mb x(t) 
% \end{align*}
% where
% \[\mb A_{(l,\tau)} =\sum_{k=1}^{\tau-1}
% \Big(\big (\mb R_1(\mb I - \mb F^*)\big)^{k-1}\Big)'
% \Big(
% (\mb q_1 + \mb F^{*'}\mb q_2) \mb F_{(l,\tau-k)}^*
% + \mb F_{(l,\tau-k)}^{*'}(\mb q_1' + \mb q_2 '\mb F^{*})
% \Big)
%   \Big(\big (\mb R_1(\mb I - \mb F^*) \big)^{k-1}\Big)
% \]
% Therefore, the linear  equilibrium is characterized by the following set of fixed point
% equations:
% \begin{align*}
%   \left\{
%     \begin{array}[]{ll}
%       \mb F_{(l,\tau)}^* = \mb e_{(l,\tau)}'
%       & \tx{if } \tau=1;
%       \\
%       \mb F_{(l,\tau)}^* = \frac{\mb e_{(l,\tau)}'\mb R_1' \mb A_{(l,\tau)}
%         \Big(\mb R_1(\mb I - \mb F^*) + \mb R_1\mb e_{(l,\tau)}\mb F_{(l,\tau)}^* \Big)
%         - \Big(\mb q_1' + \mb q_2'(\mb F^*-\mb e_{(l,\tau)}\mb F_{(l,\tau)}^*) \Big)}
%       {\mb e_{(l,\tau)}'\mb R_1' \mb A_{(l,\tau)} \mb R_1\mb e_{(l,\tau)}  + 2 \mb e_{(l,\tau)}'\mb
%         q_2}
%       &\tx{otherwise }.
%     \end{array}
%     \right.
% \end{align*}
% Can show that it is contraction mapping.  -->

\message{ !name(general_L_pricing_section1.tex) !offset(-407) }

